Wukong: A Scalable and Locality-Enhanced Framework for Serverless Parallel Computing

Serverless computing is increasingly being used for parallel computing, which have traditionally been implemented as stateful applications. Executing complex, burst-parallel, directed acyclic graph (DAG) jobs poses a major challenge for serverless execution frameworks, which will need to rapidly scale and schedule tasks at high throughput, while minimizing data movement across tasks. We demonstrate that, for serverless parallel computations, decentralized scheduling enables scheduling to be distributed across Lambda executors that can schedule tasks in parallel, and brings multiple benefits, including enhanced data locality, reduced network I/Os, automatic resource elasticity, and improved cost effectiveness. We describe the implementation and deployment of our new serverless parallel framework, called Wukong, on AWS Lambda. We show that Wukong achieves near-ideal scalability, executes parallel computation jobs up to 68.17x faster, reduces network I/O by multiple orders of magnitude, and achieves 92.96% tenant-side cost savings compared to numpywren.

==> __eval_backup_0422_12am.tex <==
\vspace{-6pt}
\subsection{End-to-End Performance Comparison}
\label{subsec:e2e}
\vspace{-2pt}

%\bencomment{New}
\noindent\textbf{Tree Reduction.} We first compared the performance of TR executing within {\proj} and Dask {\small\texttt{distributed}}~\cite{dask_distributed} (which we refer to simply as "Dask"). In our experiments, the size of the array used for TR was 1024. Additionally, we added a delay to each task of TR. We varied the amount of delay over the range of values 0~ms, 100~ms, 250~ms, and 500~ms, with 0~ms as the base case. This delay serves to simulate an increased amount of work being performed per task. 

%\noindent\textbf{Tree Reduction.} We first compared the performance of TR executing within {\proj} and Dask {\small\texttt{distributed}}~\cite{dask_distributed} (in short Dask). 
%TR serves as a microbenchmark, illustrating the types of workloads that are a good fit for \proj as well as those that are not. 
%In our experiments, the size of the array used for TR was 1024. Additionally, we added a delay to each task of the workload. We varied the amount of delay over the range of values 100~ms, 250~ms, and 500~ms, with 0~ms as a base case. 

Figure \ref{fig:tr-eval} shows that both configurations of Dask outperform {\proj} by a large margin for the base case. This is because the DAG for this workload has $1024 / 2 = 512$ leaf tasks, and each task within the workload performs a simple add operation. {\proj} immediately scales to \(512\) Lambda functions to execute the workload; however, due to the simplicity of the individual tasks, the overhead of scaling out to 512 Executors outweighs the actual benefit of the large amount of parallelism. \yuecomment{less parallelism is not true for Dask 1,000 worker config, so we need to provide better explanation.} Since Dask has less parallelism, it performs better than {\proj} for this workload.

As we add increasing amounts of delay to each TR task, we see the performance gap between Dask and {\proj} decrease. Once the delay is 250~ms or more, {\proj} executes the workload faster than the $1,000$-worker Dask cluster. 
%The delays represent additional work being done per-task. 
As the computation done by each task increases, the high parallelism of {\proj} enables the framework to achieve better performance. 
The results of this microbenchmark help to illustrate the types of workloads that benefit from execution on {\proj}. That is, {\proj} performs best when each task performs a non-trivial amount of work, as this compensates for the overhead of spinning up additional AWS Lambda functions. 

\noindent\textbf{SVD.} The results of our SVD tests demonstrate \proj's ability to provide competitive performance with traditional serverful parallel computing frameworks, while also scaling effectively for increasingly large problem sizes. 

We tested seven problem sizes for SVD1, beginning with \(128k \times 100\) (Figure~\ref{fig:svd1-eval}). We doubled the first dimension of the input matrix for each test, ending with a problem size of \(8,192,000 \times 100\). For all problem sizes, {\proj} out-performed the $1,000$-worker Dask cluster, completing the job anywhere from 62.02\% to 69.09\% faster than Dask. This performance difference results from the benefits of {\proj}'s decentralized scheduling techniques, which greatly reduce the overhead of executing tasks on a large number of workers. 
%
The Dask cluster of 125 16-core VMs consistently out-performed {\proj} for SVD1. This is because each Dask worker is provisioned with more resources, which significantly increases data locality and reduces cross-worker communications.
%likely due to the higher network bandwidth of the EC2 virtual machines in which the Dask workers are running in combination with the fact that using more powerful, multicore CPUs allows the Dask workers to complete computations more quickly than {\proj} workers.

%For the first half of the tests, the communication delay from transferring code and data outweighed the increased parallelism provided by {\proj}. As we increased the problem sizes however, {\proj} began to outperform Dask. At first, the performance difference was small, with {\proj} completing the job roughly 6.2\% faster on average for the \(2,048,000 \times 100\) problem size. This difference increased to 29\% for the \(4,096,000 \times 100\) case and  44.6\% for the largest problem size.

%\yuecomment{Suggest that we  remove SVD2 as it repeats what we saw for SVD1.} \bencomment{Yeah, if we need something to cut, then we can likely remove SVD2; however, SVD2 is one of the largest problem sizes we show results for (256k x 256k for SVD is relatively complicated/large).}
For SVD2, we observe similar trends in performance. For smaller problem sizes, {\proj} was not able to out-perform either configuration of Dask due to the overhead of performing I/O. As the problem size increased however, the benefit of {\proj}'s increased parallelism and decentralized scheduling enabled it to out-perform the 1,000-node Dask cluster. Further, {\proj} was able to scale to considerably larger problem sizes than the 1,000-node Dask cluster. As with SVD1, the 125-node Dask cluster out-performed {\proj} by a considerable margin. This is once again due in part to the increased network bandwidth and more powerful processors used by the Dask workers.
%we also tested seven different problem sizes. 
%the first half of tests included smaller-scale matrices while the second half included medium-to-large scale matrices. Looking at Figure \ref{fig:svd2-eval}, we can see that {\proj}'s performance was worse than Dask for smaller problem sizes. This is once again due to the communication delay associated with transferring data. Once we increased the problem size to larger matrices, {\proj} began to outperform Dask by a small margin. 
%Specifically, {\proj} executed the workload 9.53\% and 7.85\% faster than Dask for \(100k \times 100k\) and  \(128k \times 128k\) matrices, respectively.
%The performance gap between the two frameworks decreased as the problem sizes increased, falling to just 8.22\% for \(100k \times 100k\) matrices and 4.78\% for \(128k \times 128k\) matrices. 
%As we further increased the problem size to \(192k \times 192k\), {\proj} was able to scale far more effectively, executing the workload 3.2\(\times\) faster than Dask {\small{\texttt{distributed}}}. Lastly, {\proj} was able to complete the largest problem size of \(256k \times 256k\) while Dask was unable to do so due to out-of-memory errors. 

%\yuecomment{}
%Finally, we compared the performance of {\proj} against that of numpywren~\cite{numpywren}, a state-of-the-art serverless execution platform for linear algebra. We were unable to install and run numpywren ourselves, so we compared the {\proj} results against the SVD results reported in \cite{numpywren}. Specifically, we used the results of {\proj} running SVD2, as this is the closest equivalent to numpywren's SVD tests. As shown in Figure~\ref{fig:svd2-numpywren-eval}, numpywren calculated the SVD of a \(256k \times 256k\) matrix in 77,828 seconds while {\proj} computed this result in 88.19 seconds using the DAG generated for Dask's SVD implementation with a square matrix. These results show \proj's elasticity and its ability to deliver competitive performance, even at larger scales. 

%\bencomment{New}
\noindent\textbf{SVC.} Figure~\ref{fig:svc-eval} shows the performance on SVC. We compared the performance of {\proj} and Dask on eight different problem sizes, ranging from $128k$ to $16.3M$ samples. To create the input DAGs for {\proj}, we used Dask-ML's {\small{\texttt{ParallelPostFit}}} library~\cite{dask_ml_ppf}. As with the previous benchmark, Dask was able to perform better for smaller problem sizes; however, when we increased the problem size, the performance gap between the two frameworks decreased. Beginning with the \(256 k\) problem size, Dask tended to outperform {\proj}. As the scale of the problems increased to $4.0M$ samples and beyond, {\proj} began to scale more effectively than the $1,000$-worker Dask cluster. The large parallelism of {\proj} enabled the framework to complete the workload in 46.45\% less time. The performance difference between {\proj} and the $125$-worker Dask cluster was similar, with Dask executing the workload roughly 50.56\% faster than {\proj}.

%\bencomment{New}
\noindent\textbf{GEMM.} Like TR, the results of our GEMM experiments identify a  workload that is difficult to execute in a serverless environment. As shown in Figure~\ref{fig:gemm-eval}, we tested GEMM across five different problem sizes. In all except the largest test, {\proj} achieved significantly worse performance than Dask. This is because the GEMM implementation requires a number of relatively large intermediate objects to be communicated between tasks before the computational portion of the workload can begin. Due to the limited bandwidth available to the AWS Fargate nodes and the AWS Lambda functions, {\proj} experiences long delays during this phase of the workload. It isn't until the largest problem size that the increased parallelism of {\proj} enables it to achieve comparable performance to Dask. 

While {\proj} was only able to roughly match Dask's performance for GEMM, {\proj}'s performance greatly exceeded that of both numpywren configurations for problem sizes \(5k \times 5k\) to \(15k \times 15k\). For the largest problem size, {\proj} (with a single Redis shard) executed the workload 89.76\% faster than numpywren (with a single Redis shard). {\proj} (with Fargate) was 51.22\% faster than numpywren (with S3) for $15k \times 15k$ problem size, likely because {\proj}'s Fargate KVS layer achieves lower latency compared with AWS S3.
%While numpywren with S3 was 18.82\% faster than {\proj}, this is likely due to the fact that S3 can perform better for a workload like GEMM while Redis experiences considerable performance degradation. 

\input{scalability_eval_fig}

%\yuecomment{FIXME: would suggest removing the next para, and only keep the para after the next.}
%As it is currently implemented, GEMM is unable to benefit from clustering and delay scheduling. This is due to the DAG structure of the GEMM workload as generated by Dask. The leaf task layer is composed exclusively of tasks that produce large objects, while the second layer is the matrix-multiplication tasks (i.e., tasks whose code is responsibility for carrying out the matrix multiplication operation). Each matrix multiplication task in the second layer depends on multiple leaf tasks and therefore multiple big input objects. Clustering and I/O delays do not produce a significant benefit for situations in which a single task depends on many large objects as there is no way for these optimizations to remove all of the large object I/O without also removing all of the parallelism. 
%\bencomment{I believe I removed the paragraph you suggested.}
%\yuecomment{This para is enough to explain the performance issue of GEMM.}
Note that task clustering and delayed I/O is not effective for GEMM due to its simple DAG structure (see Figure~\ref{fig:gemm}). Each large object in GEMM is used as input for a (possibly large) number of downstream tasks. In order to cluster tasks so that all large object I/O would be removed, much of the workload would need to be clustered onto the same Lambda function. In testing, this produced significantly longer execution times for GEMM workloads due to the loss of parallelism. Again, coarser execution (possibly 8 or 16 core Lambdas with more memory) wins, which is not possible for current serverless platforms.



%\bencomment{New}
\noindent\textbf{TSQR.} For the first two problem sizes, both Dask clusters outperformed {\proj} and numpywren. Beginning with the \(131,072 \times 128\) matrix, {\proj} matched the $1,000$-worker Dask cluster's performance. As the problem sizes increased, {\proj} began to outperform this Dask cluster. This gap increased gradually up through the problem size \(4,194,304 \times 128\), at which point {\proj} began to outperform the $1,000$-worker Dask cluster by increasingly significant margins. 
By the largest problem size, {\proj} was completing the workload $92.35\%$ faster than $1,000$-worker Dask. 

\yuecomment{Make sure to compare wukong redis with numpywren redis and wukong fargate with numpywren s3 for fairness. }
{\proj} outperformed both numpywren (with S3) and numpywren (single Redis shard) for all problem sizes. For the \(4,194,304 \times 128\) matrix, {\proj} (single Redis shard) was executing the workload \(68.17\times\) faster, or in 98.53\% less time, than numpywren (single Redis shard); and {\proj} (Fargate) is \(35.62\times\) faster, or in 97.19\% less time, than numpywren (S3). Numpywren (single Redis shard) failed to execute the next larger problem size, and the last workload numpywren (S3) was able to execute was \(16,777,216 \times 128\). For this workload, {\proj} was \(11.25\times\) faster, executing the workload in $91.11\%$ less time.

%The 125-worker Dask cluster was considerably faster than all other frameworks and configurations, completing the workload in 37.27\% less time than {\proj}.

\vspace{-4pt}
\subsection{Scalability and Elasticity}
\label{subsec:e2e}
\vspace{-2pt}

We next evaluate the  scalability and elasticity of {\proj}'s compute and storage substrates. The compute substrate consists of {\proj}'s static scheduler and the AWS Lambda Task Executors. The storage substrate is composed of an AWS Fargate Cluster in which each node is running an instance of Redis as well as an EC2 VM that hosts both a KV Store Proxy and another instance of Redis. The EC2-hosted Redis instance is used exclusively for storing static schedules, dependency counters, and final results.

\begin{comment}
\yuecomment{I commented it out for now if it repeats what we have said before.}
\bencomment{Not sure if this brief re-explanation of storage manager is necessary here or not.}
By using AWS Fargate as its storage medium instead of AWS Elasticache, {\proj} gains both storage level elasticity and cost effectiveness without sacrificing performance. Even though AWS Fargate nodes are elastic resources, their performance is still competitive, particularly for very small and very large objects.
\end{comment}

\noindent\textbf{Strong Scaling.} Figure~\ref{fig:scalability} shows the strong and weak scaling behavior of {\proj}. In order to test the strong scaling of {\proj}, we varied the number of workers used to execute a workload of $10,000$ tasks. In order to simulate more complicated workloads, we repeated the experiment three times, adding a delay of 100~ms, 250~ms, and finally 500~ms to each task. 

The expected ideal curve is shown as a black dashed line, while {\proj}'s strong scaling is shown in blue and Dask's strong scaling is shown in green. In all cases, {\proj} exhibited near-ideal strong scaling behavior, scaling significantly better than Dask for 0~ms delay, thereby demonstrating the effectiveness of our decentralized scheduling mechanism. As the delay added to each task increased, Dask's scaling behavior quickly approached that of {\proj}.

\noindent\textbf{Weak Scaling.}
To test {\proj}'s weak scaling behavior, we executed ten tasks per worker and varied the number of workers from 20 to 320. Just as with our strong scaling experiments, we also added an equal amount of delay to each task, and we varied the length of the delay using the values 100, 250, and 500~ms. While Dask performed better than {\proj} for 20, 40, and 80 workers, {\proj} scaled significantly better than Dask for 160 workers and beyond. This behavior is primarily due to {\proj}'s decentralized design, which enables the framework to scale to large numbers of workers without a significant increase in overhead. 
%\bencomment{{\proj} scaled better than Dask for 160+ workers for 0ms and 100ms. But for 250ms and 500ms, {\proj} scaled "significantly" better for just 320 workers. Do we need to adjust how we describe the scaling based on that?} \yuecomment{We can add one or two sentences to justify why ABC scales better than Dask for larger number workers.}
%even better for 320 workers. 
In addition, {\proj} exhibited near-ideal weak scaling behavior, as shown by the dotted black line. Finally, as the length of the delay added to each task increased, the difference in weak scaling behavior between Dask and {\proj} decreased for both small and large worker cluster sizes. 








\begin{comment}
%% yue: comment out the following Fargate eval... 
%\yuecomment{I suggest we remove the eval for Fargate storage.}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.38\textwidth]{Plots_v3/ABC_vs_Elasticache.pdf}
\vspace{-10pt}
\caption{Timeline of launching 100 Fargate and ElastiCache.}
\vspace{-15pt}
\label{fig:abc_vs_elasticache_elasticity}
\end{center}
\end{figure}

\noindent\textbf{Intermediate Storage Elasticity.} 
Figure~\ref{fig:abc_vs_elasticache_elasticity} shows the number of Fargate Redis nodes launched by {\proj}'s storage substrate vs. AWS ElastiCache {\small{\texttt{cache.m4.2xlarge}}} nodes over time. {\proj}'s storage substrate provisioned 100 nodes in approximately 475~seconds (7.92~minutes) while AWS Elasticache took approximately 795~seconds (13.25~minutes) to provision the same number of nodes. In addition, the storage substrate provisioned 85 nodes in 260 seconds while Elasticache took 650 seconds to provision the same number of nodes. {\proj} provisioned 85 nodes \(2.5\times\) faster and 100 nodes \(1.67\times\) faster than AWS Elasticache. Notably, scaling out to 20 nodes takes about 100 seconds; in practice, 20 Fargate nodes should be sufficient for most (if not all) application scenarios (as will be shown in Figure~\ref{fig:svd2-fargate-nodes-vs-runtime}) if task clustering and delay I/O are enabled.

%\rickcomment{It is not clear why you are comparing Fargate to Elasticache and Ec2 Redis. When you say "AWS Elasticache or EC2", do you mean that you ran ABC's workloads with storage implemented using Fargate and you ran the same workloads with ABC storage implemented using AWS Elasticache and with EC2, and you are comparing the results to show ABC with Fargate is the best implementation? } \bencomment{Yes, we're essentially showing that AWS Fargate provides the best medium for hosting the storage substrate. We want to show that (1) it provides sufficient performance, (2) it is sufficiently scalable/elastic, and (3) it is cost-effective.}

\begin{figure}[t]
%\vspace{-5pt}
\begin{center}
\subfigure[Small reads.] {
\includegraphics[width=0.23\textwidth]{Plots_v3/FargateVsEC2_Reads_Small.pdf}
\label{fig:small_reads}
}
\hspace{-16pt}
\subfigure[Large reads.] {
\includegraphics[width=0.23\textwidth]{Plots_v3/FargateVsEC2_Reads_Large.pdf}
\label{fig:large_reads}
}
%\hspace{-8pt}
\subfigure[Small writes.] {
\includegraphics[width=0.23\textwidth]{Plots_v3/FargateVsEC2_Writes_Small.pdf}
\label{fig:small_writes}
}
\hspace{-16pt}
\subfigure[Large writes.] {
\includegraphics[width=0.23\textwidth]{Plots_v3/FargateVsEC2_Writes_Large.pdf}
\label{fig:large_writes}
}
\vspace{-15pt}
\caption{Performance of ElastiCache (EC) vs. Fargate.}
\label{fig:fargate_lat}
\vspace{-15pt}
\end{center}
\end{figure}

\noindent\textbf{Intermediate Storage Performance.} Next, we compare I/O latency for Fargate-based Redis against AWS ElastiCache {\small{\texttt{m4.2xlarge}}} instances. Figures \ref{fig:fargate_lat} shows the read and write latencies for varying the object sizes. Fargate-hosted Redis instances provide  comparable performance for read and write operations on data that is 1MB or smaller. For small reads of 256 bytes, 1~kB, and 256~kB, Fargate achieves lower latencies than ElastiCache-hosted Redis. 
%As the size of the data increases to 16MB, 32MB, and 64MB, the lower bandwidth of AWS Fargate results in longer latencies for both read operations and write operations. 
For the largest sizes tested (128~MB and 256~MB), Fargate and ElastiCache showed near-identical latencies for both read and write operations.  
%\bencomment{TODO: Make sure wording for this and previous paragraph is okay.}%\bencomment{We need to say machine type for ElastiCache? We did benchmarks on EC2, but in theory the performance between EC2 and ElastiCache should be the same.} \yuecomment{We can use m4.2xlarge as it provides the same amount of memory. }
\end{comment}






\vspace{-5pt}
\subsection{Factor Analysis}
\label{subsec:factor}
\vspace{-3pt}




Finally, we discuss the results of our factor analysis of {\proj}. 
%At a high level, our analysis demonstrates the importance of selecting an appropriate data partition size in order to achieve the best performance. Similarly, our analysis shows how the performance of {\proj} scales with the number of nodes in the AWS Fargate cluster. 

\noindent\textbf{Partition Size.} 
The partition size of input data is one of the most important configuration parameters when executing a workload on {\proj}. This parameter controls how the input data is divided and subsequently processed, and presents an interesting tradeoff. Specifying a large partition size results in less parallelism and high network bandwidth consumption.
%as in a small number of coarse-grained tasks, 
%and very large data sizes for network I/O operations. 
On the other hand, specifying a small partition size may generate too many fine-grained tasks, resulting in a very large number of individual connections between Task Executors and the storage cluster as well as very small data sizes for network I/O operations. Consequently, it is necessary for the user to find a balance in order to achieve optimal performance. The optimal value of the partition size will change depending on the application type and problem size. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.38\textwidth]{Plots_v3/SVD2_PartitionSizeVsRuntime.pdf}
\vspace{-15pt}
\caption{
%SVD2 partition size vs. execution time.
SVD2 execution time as a function of the partition size.
}
\vspace{-10pt}
\label{fig:svd2-partitions-vs-runtime}
\end{center}
\end{figure}

Figure~\ref{fig:svd2-partitions-vs-runtime} shows the performance of SVD2 with a problem size of \(50k \times 50k\) for various partition sizes. Selecting a small partition size such as \(2k \times 2k\) causes significant network contention resulting from too many individual connections and I/O operations. Increasing the partition size alleviates this contention and improves overall performance. Notice that continuing to increase the problem size for SVD2 does not impact performance significantly. Instead, the performance will remain approximately the same as the partition size increases.  This is because task clustering and delayed I/O prevent network communication of large objects. That is, increasing the partition size does not impact the workload significantly once clustering and delay I/O are in effect.
%\bencomment{Should we provide an explanation for this trend?} \yuecomment{I feel we need to add a short sentence to explain it.}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{Plots_v3/SVD2_NumFargateNodesVsRuntime.pdf}
\vspace{-10pt}
\caption{
SVD2 performance and the I/O latencies when varying the Fargate cluster size.
%SVD2 number of Fargate nodes vs. runtime
}
\vspace{-15pt}
\label{fig:svd2-fargate-nodes-vs-runtime}
\end{center}
\end{figure}

\noindent\textbf{Number of Storage Nodes.} Next, we evaluate how the number of nodes in the storage substrate impacts execution time. Figure~\ref{fig:svd2-fargate-nodes-vs-runtime} shows the performance of SVD2 with a problem size of \(128k \times 128k\) for different numbers of Fargate nodes, along with the associated average read and write latencies for each configuration. Using a small number of nodes such as 5 or 10 results in significant performance degradation, as the limited number of Redis instances suffer severe network bandwidth contention. As we increase the size of the Fargate cluster, read latencies decrease significantly, resulting in a lower execution time for the workload.

Execution time will no longer decrease once the number of Fargate nodes increases beyond a certain threshold. The value of this threshold is predominantly dependent on problem size, as a larger problem size would benefit from a larger number of Fargate nodes compared to a smaller problem size. 
%\bencomment{What to say about write latencies?}  

\noindent\textbf{Task Clustering and Delay I/O.} Finally, we look at the impact of task clustering and delaying I/O on {\proj}'s performance.
%how each individual task is processed. 
Clustering and delay I/O prevent tasks with large intermediate data from writing their data to Redis. Instead, these tasks attempt to execute downstream tasks locally. Any downstream tasks that cannot immediately be executed because their dependencies are not satisfied are put into a queue. The  dependencies of the queued tasks are routinely rechecked until the dependencies are satisfied or a maximum delay time is reached. By delaying I/O, more tasks can be clustered and expensive network I/Os data can be avoided, decreasing the workload runtime dramatically. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{Plots_v3/SVD50k_Clustering_vs_NoClustering.pdf}
\vspace{-10pt}
\caption{
SVD2 50k x 50k aggregated execution time breakdown with and without task clustering and delay I/O.
%Impact of task clustering and delay I/O on the performance of SVD $50k \times 50k$.
}
\vspace{-15pt}
\label{fig:svd-cluster-vs-no-cluster}
\end{center}
\end{figure}

%\yuecomment{FIXME: Note to be consistent, I replaced all ``I/O delays'' with ``delay I/O''. Design section might also need this change.}
Figure~\ref{fig:svd-cluster-vs-no-cluster} displays two aggregations of time for the activities performed during the processing of tasks. 
%Specifically, the top bar shows the aggregated time breakdown of the activities performed during SVD2 \(50k \times 50k\) with clustering and delayed I/O disabled, while the bottom bar shows the breakdown for the same benchmark with clustering and delayed I/O enabled. 
In both cases, ``publishing messages'', ``task execution'', and ``serialization/deserialization'' each took approximately the same amount of time (in aggregate); however, the difference between the times for task invocation and especially Redis I/O is significant. With the two optimizations disabled, task invocations and Redis I/O made up an aggregate 14.80 and 565.21 seconds, respectively. When the optimizations were enabled, task invocation took an aggregate 2.05 seconds while Redis I/O took just 20.36 seconds. That is, there is \(7.21\times\) more aggregate time spent invoking tasks and \(27.76\times\) more aggregate Redis I/O performed with clustering disabled. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.35\textwidth]{Plots_v3/ABCOptimizations_BarGraph.pdf}
\vspace{-10pt}
\caption{
%Performance of {\proj} with the inclusion of each major optimization.
Contributions of major optimizations to {\proj}'s performance.}
\vspace{-15pt}
\label{fig:abc-optimizations}
\end{center}
\end{figure}

%\bencomment{Wrote paragraph for Figure \ref{fig:abc-optimizations}. Replaced old paragraph with this new one. Old paragraph was not necessary imo.}

%Figure~\ref{fig:abc-optimizations} shows how the performance of SVD2 \(100k \times 100k\) changes depending on the optimizations used.
We analyze {\proj}'s performance by breaking down the performance gap between a baseline and {\proj} with all optimizations enabled (see Figure~\ref{fig:abc-optimizations}).
The use of the Fargate storage cluster results in a 20.85\% performance improvement over using AWS ElastiCache for intermediate data storage. When using Fargate, the I/O performed during the workload is spread across a large number of Redis instances, resulting in reduced network contention and consequently reduced I/O latency. (Using a large number of AWS ElastiCache instances is cost prohibitive.) When clustering (without delayed I/O) is enabled, performance improves by another 48.82\% as a significant amount of large object I/O is eliminated from the workload. Finally, enabling delayed I/O results in a 46.21\% improvement relative to the use of clustering and Fargate alone. Overall, {\proj} is 4.6$\times$ faster when all major optimizations are used, demonstrating the effectiveness of the optimization techniques.



%\yuecomment{FIXME: the following para seems not related to Figure~\ref{fig:abc-optimizations}, which needs a para.}
%In order to achieve optimal performance, it is necessary to use both delayed I/O and task clustering. That is, delayed I/O can significantly improve the performance of a workload that is already using clustering. For example, the use of delayed I/O (in addition to task clustering) results in a 46.21\% speedup for SVD2 \(100k \times 100k\) compared to using clustering without delayed I/O. In general, workloads that benefit from task clustering will also benefit from delayed I/O, especially as the problem size increases. delayed I/O and task clustering together can potentially eliminate large object I/O entirely, thereby removing one of the most significant bottlenecks from the workload's execution. Lastly, delayed I/O have benefits beyond strictly improving performance in that it can significantly reduce costs. This will be discussed in-depth in the next section. 

\vspace{-6pt}
\subsection{Monetary Cost}
\label{subsec:e2e}
\vspace{-3pt}

{\proj} takes advantage of AWS Lambda's pay-per-use pricing model to keep costs\footnote{Note the ``cost'' here refers to cloud tenant-side monetary cost.} low while still providing competitive performance. We now analyze the difference in cost between running a workload on serverful Dask compared to serverless {\proj}.

%\bencomment{The following sentence originally said "Recall the two setups..." but since we don't use the same setup for {\proj}, I changed the sentence slightly: }
\bencomment{This needs to be updated.} Recall the Dask setup from the benchmarks discussed above. Dask {\small\texttt{distributed}} ran on an 11-node cluster of {\small{\texttt{r5.4xlarge}}} EC2 VMs. According to Amazon's EC2 On-Demand price listings~\cite{aws-on-demand-pricing}, a single {\small{\texttt{r5.4xlarge}}} instance costs \$1.008/hour. Therefore, the cost of running eleven of these instances is approximately \$11.09/hr. 

\noindent\textbf{Total Cost.} In order to analyze the cost trade-off between Dask and {\proj}, we use the SVD2 \(128k \times 128k\) benchmark as a sample. With 25 Fargate nodes, two {\small{\texttt{c5.12xlarge}}} EC2 VMs, and the AWS Lambda Task Executor configured to use 1024~MB of memory, {\proj} is able to execute this workload in 23.84 seconds while Dask completes this workload in 21.54 seconds if configured as described above. The cost of executing this workload on Dask is calculated as
%is equal to the CPU time multiplied by the cost of running the cluster for an hour. Since EC2 charges to the nearest minute, we round up the execution time of 21.54 seconds to one minute. With this, the cost of running the Dask cluster is equal to 
%\(11 EC2 VMs \times \$1.008 \times 0.16667 hours\) or 
\$0.1848. 
%\bencomment{Note that I have configured {\proj} differently than what we used for the other benchmarks. This is because the configuration I am using here is most cost-effective while still providing competitive performance. Should we explicitly state that we altered {\proj}'s configuration here for the purposes of cost-effectiveness?}
%\yuecomment{I think it's OK to alter it without mentioning it. It is a lot of details. }

In the case of {\proj}, we must consider the cost of running the nodes in the Fargate storage cluster~\cite{aws-fargate-pricing} (25 nodes cost \$0.014764), the EC2 instances (two {\small{\texttt{c5.12xlarge}}} cost \$0.068) for the Static Scheduler and KV Store Proxy, and the cost of executing the AWS Lambda functions. 
%Pricing information for AWS Fargate is available online on the AWS website \cite{aws-fargate-pricing}. 
%In this case, the Fargate cluster was composed of 25 nodes, each configured to have 4 vCPUs and 30GB RAM. Based on this, the total cost of running the Fargate cluster is approximately \$0.014764. Next, running two {\small{\texttt{c5.12xlarge}}} instances costs approximately \$4.08/hour. We round up the execution time from 22.75 seconds to 1 minute to calculate the cost for EC2. In this case, running the two EC2 virtual machines cost approximately \$0.068.
%
%Finally, t
%\bencomment{Do we want to state the aggregate duration as 10,089 seconds given how long that is?}
%The aggregate duration of the Lambda functions used during the workload was 10,089 seconds. 
AWS Lambda charges function usage to the nearest 100~ms. For 1~GB Lambdas, the cost per 100~ms is \$0.000001667~\cite{aws-lambda-pricing}. Using this information, the cost of executing the Lambda functions was approximately \$0.1188. All together, the cost of running {\proj} was \$0.201595 for SVD2 \(128k \times 128k\). This is just \$0.016795 more than the cost of executing the workload on Dask. 

Notably, AWS Lambda constitutes 58.93\% of the total cost of the workload, and tenants are only charged for Lambda while the workload is running. It is important to note that for serverful deployments, tenants are billed before and after the workload executes, i.e., when the servers are not being utilized, at the same rate as when the workload is actively executing. As a result, the cost of {\proj} is considerably less than serverful alternatives, such as Dask, when utilization is factored into the price.

%\bencomment{In the next two paragraphs, I am wondering if it sounds more impactful to say "the workload is X$\times$ cheaper" or "reduces the cost by X\%". See my comments. Additionally, if we use "X$\times$", then I believe the wording should probably be changed slightly (i.e., "workload costs X$\times$ less" or "is X$\times$ cheaper").}

\noindent\textbf{Impact of Optimizations on Cost Saving.} Task clustering and delayed I/O are key optimizations, not only for increasing the performance of {\proj}, but for reducing the overall cost as well. The degree to which these optimizations reduce workload cost increases with problem size, just as their impact on performance does. For example, the use of task clustering and delayed I/O  decreases the cost of running 3~GB Lambda task executors in SVD2 \(50k \times 50k\) by approximately 65.23\% (from \$0.04556 to \$0.01584). 

This effect on cost is even more pronounced for larger problem sizes. For SVD2 \(100k \times 100k\), the cost of running 3~GB Lambda task executors with task clustering enabled and delayed I/O \textit{disabled} is approximately \$1.17. When delay I/O is enabled, the cost of executing 3~GB Lambda task executors drops to just \$0.31. That is, the use of delay I/O reduces the cost of the workload by 73.50\%.
%for a workload of this size. 
This is because delayed I/O coupled with task clustering almost entirely eliminates large object I/Os, while clustering alone simply reduces the frequency of such operations. 

\noindent\textbf{Storage Cost.} We analyze the cost efficiency of {\proj}'s storage substrate. Consider a 50-node Fargate cluster in which each node is configured to have 4 vCPU and 30~GB of memory. The cost-per-hour of this cluster would be determined by both the ``per vCPU per hour'' and ``per GB per hour'' cost dimensions~\cite{aws-fargate-pricing}.
%as described on Amazon's website \cite{aws-fargate-pricing}. 

Note that by default, {\proj} is configured to use Fargate Spot as its capacity provider, so we will use that pricing model in these calculations \bencomment{(We were criticized for using Fargate Spot pricing here and non-spot pricing for Dask. But it is hard to get enough spot instances (that aren't shut down mid-execution) to host Dask cluster. Also, Fargate Spot allows up to 250 Fargate nodes while non-spot only allows up to 100)}. Based on the information online, the ``per vCPU per hour'' cost dimension would be equal to 4 vCPU $\times$ \$0.012144 $\times$ 1 hour $\times$ 50 nodes, or \$2.4288. The ``per GB per hour'' dimension would be equal to 30GB $\times$ \$0.0013335 $\times$ 1 hour $\times$ 50 nodes or approximately \$2.00025. Taking the sum of these two values, we obtain the cost of running this Fargate cluster: \$4.43 an hour. 

If we were to instead use a 50-node EC2 cluster of virtual machines with similar specs (e.g., {\small{\texttt{r5.xlarge}}} with 4 vCPU and 32GB memory), the cluster would cost \$12.6 per hour. Alternatively, if we were to use AWS ElastiCache~\cite{aws-elasticache-pricing}, we could run a cluster of 50 {\small{\texttt{cache.r5.xlarge}}} nodes. Each {\small{\texttt{cache.r5.xlarge}}} has 4 vCPU,  26.32~GB memory, and costs \$0.431 per hour. Therefore, a 50-node cluster of {\small{\texttt{cache.r5.xlarge}}} nodes would cost \$21.55 per hour. Based on this, {\proj}'s lightweight storage substrate costs $64.8\%$ less than AWS EC2 and $79.4\%$ less than AWS ElastiCache, respectively.
%Based on this, {\proj}'s storage substrate costs 90.27\% less than AWS EC2 and %2.84$\times$ cheaper than AWS EC2 and %4.86$\times$
%96.11\% less than AWS ElastiCache. 
%\bencomment{Changed 2.84x and 4.86x to 90.27\% and 96.11\%, respectively.}

==> _moti_atc.tex <==
\section{Motivation}
\label{sec:moti}



The design of {\proj} was motivated in part by the dominance of network IO during workload execution. The three key innovations of decentralized scheduling, task clustering, and the elastic storage layer each address a different aspect of the challenges presented by managing network IO in a serverless context. 

First, we consider the characteristics of the intermediate data generated during the execution of a workload on {\proj}. Figure \ref{fig:svd2-io-cdf} presents a CDF of the sizes of objects read and written during the execution of SVD with input size \(50k \times 50k\). From this graph, it is clear that the workload is heterogeneous with respect to the object sizes contained throughout. While a large number of reads and writes are for objects less than 1MB in size, there are a significant number of objects transferred whose size is greater than 1MB. In fact, roughly 10\% of the objects read or written during this workload were approximately 200MB in size. The wide range of object sizes presents unique opportunities for storage design. 

Next, we look at the breakdown of the total time processing each task during a workload (i.e., all of the activities performed in relation to the given task including IO, serialization, execution, etc.). Looking at Figure \ref{fig:svd2-flame}, we can see that nearly all tasks spend a majority of their time performing network-based read and write operations. The actual execution of a given task's code constitutes an extremely small percentage of the overall time spent processing the task. Based on this, it is clear that a new approach to intermediate data storage is required in order to achieve competitive performance in a serverless environment. 

Finally, we investigate the inability of a centralized scheduler to perform in a serverless environment. Figure \ref{fig:decent-sched-moti} shows the performance of a few design iterations of a naive centralized scheduler, with the right-most bar showing the performance of a \textit{decentralized} scheduler. The strawman version of {\proj} adopts a purely centralized design. This created a significant bottleneck within the centralized Scheduler, as it was unable to process and invoke tasks fast enough to out-perform traditional, purely-serverful DAG schedulers. 

The performance boost gained by using multiple processes to invoke tasks in parallel, as shown by the second bar, was far from enough. While tasks could now be invoked more rapidly, the bottleneck of processing the tasks within the Scheduler still existed. Using a more efficient messaging service in that of Redis Pub/Sub over the use of direct TCP connections further improves performance, but the main underlying bottleneck still persists. It was not until a decentralized scheduling design was adopted that performance improved considerably. The burden of scheduling tasks is spread across all of the workers (which are AWS Lambda functions), eliminating the previous bottleneck.  

==> abstract.tex <==
\vspace{-15pt}
\begin{abstract}
\vspace{-10pt}
%Serverless computing is increasingly being used for parallel computing, which have traditionally been implemented as stateful applications. 
Executing complex, burst-parallel, directed acyclic graph (DAG) jobs poses a major challenge for serverless execution frameworks, which will need to rapidly scale and schedule tasks at high throughput, while minimizing data movement across tasks. We demonstrate that, for serverless parallel computations, decentralized scheduling enables scheduling to be distributed across Lambda executors that can schedule tasks in parallel, and brings multiple benefits, including enhanced data locality, reduced network I/Os, automatic resource elasticity, and improved cost effectiveness.
We describe the implementation and deployment of our new serverless parallel framework, called {\proj} (Locality-Aware, Decentralized Serverless scheduling), on AWS Lambda. We show that {\proj} achieves near-ideal scalability, executes parallel computation jobs up to $68.17\times$ faster, reduces network I/O by multiple orders of magnitude, and achieves $92.96\%$ tenant-side cost savings compared to numpywren.
%by as much as $96.40\%$.
%{\proj}  uses optimization techniques for scheduling, computing, and data storage that together overcome the bottlenecks the can arise during serverless task scheduling and network I/O. {\proj} partitions a DAG and offloads sub-graph task scheduling to a fleet of Lambda-based task executors to decentralize scheduling. {\proj} performs runtime optimization techniques to enhance data locality and reduce network I/Os.  Furthermore, {\proj} leverages a lightweight and elastic AWS Fargate-managed intermediate storage substrate to reduce storage costs without sacrificing performance. {\proj} is the first, holistic, serverless, parallel computing framework to combine all of these techniques. On AWS, {\proj} achieves near-ideal scalability, executes a wide range of parallel computation workloads up to $3.3\times$ faster than Dask, and can effectively reduce network I/O by as much as $96.40\%$.

\end{abstract}

% Working on modified abstract.

% Focus more on data, storage, data locality, minimizing network IO, etc.?

% Reworking paragraph #2
% In this paper, we identify and evaluate a set of techniques to make DAG schedulers serverless-aware. To that end, we introduce {\proj}, a serverless DAG scheduler built atop AWS Lambda and AWS Fargate. {\proj} uses decentralized scheduling through a combination of static and dynamic scheduling to provide scalable, competitive workload execution while keeping costs low. We present an empirical study in which we run and analyze a number of different applications on {\proj}. Our experimental results demonstrate the efficacy of {\proj} in minimizing the performance constraints introduced by AWS Lambda to deliver performance competitive with traditional, serverful DAG schedulers. 

% Contributions
% -------------
% Effective decentralized scheduling that significantly improve the scheduling performance and scalability (so a part of our   evaluation should focus on this);
% Smart locality-aware scheduling that improves data locality and reduces unnecessary data movement via network;
% Elastic and lightweight storage substrate (is there any shining point that we want to show to the audience?)


%This used to be at the beginning: %Compute-intensive and data-intensive applications can be modeled as and compiled into a directed acyclic graph (DAG) based workflow, where the nodes are fine-grained tasks and the edges are task dependencies. Such workflows are increasingly characterized by fine-grained burst-parallel tasks.  
%short, fine-grained tasks with large fan-outs that lead to bursts of new tasks. 
%These characteristics make them well-suited for an increasingly prevalent cloud computing model called serverless computing.
%or Function-as-a-Service (FaaS). 
%The auto-scaling property of serverless computing platforms accommodates short tasks and bursty workloads, while the pay-per-use billing model of serverless computing providers keeps the cost of short tasks low.
%Existing serverless parallel 
%Researchers have identified new use cases of serverless computing to parallelize and accelerate complex applications such as analytics and linear algebra. However, 
%However, due to the inherent data communication constraints of today's serverless platforms, it remains a challenge to harness serverless computing's massive parallelism and elasticity in high performance parallel computing applications.
%fine-grained, pay-per-use billing model in high performance parallel computing applications. 
%to realize a cost-efficient, high-performance serverless parallel computing framework.

==> cost_fig.tex <==


\begin{figure}[t]
%\vspace{-5pt}
\begin{center}
\subfigure[Total core seconds.] {
\includegraphics[width=0.23\textwidth]{Plots_v5_Drafts/SVD1_CPUComparison.pdf}
\label{fig:svd1-core-seconds}
}
\hspace{-10pt}
\subfigure[Cost comparison.] {
\includegraphics[width=0.23\textwidth]{Plots_v5_Drafts/SVD1_CostComparison.pdf}
\label{fig:svd1-cost}
}
\vspace{-10pt}
\caption{SVD1 CPU time and cost comparison.}
\label{fig:svd1_cost}
\vspace{-15pt}
\end{center}
\end{figure}

\begin{figure}[t]
%\vspace{-5pt}
\begin{center}
\subfigure[CPU usage comparison.] {
\includegraphics[width=0.22\textwidth]{Plots_v5_Drafts/GEMM_SR_vCPUs.pdf}
\label{fig:gemm_vcpu}
}
\hspace{-8pt}
\subfigure[Cost comparison.] {
\includegraphics[width=0.22\textwidth]{Plots_v5_Drafts/GEMM_SR_CumulativeCost.pdf}
\label{fig:gemm_cost}
}
\vspace{-10pt}
\caption{GEMM CPU usage and cost timeline.}
\label{fig:gemm_cost}
\vspace{-15pt}
\end{center}
\end{figure}

\begin{figure}[t]
%\vspace{-5pt}
\begin{center}
\subfigure[CPU usage comparison.] {
\includegraphics[width=0.22\textwidth]{Plots_v5_Drafts/TSQR_4M_vCPU_Combined.pdf}
\label{fig:tsqr_vcpu}
}
\hspace{-8pt}
\subfigure[Cost comparison.] {
\includegraphics[width=0.22\textwidth]{Plots_v5_Drafts/TSQR_4M_CostCombined.pdf}
\label{fig:tsqr_cost}
}
\vspace{-10pt}
\caption{TSQR CPU usage and cost timeline.}
\label{fig:tsqr_cost}
\vspace{-15pt}
\end{center}
\end{figure}










% commented out old fig...
\begin{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\begin{minipage}[b]{0.23\textwidth}
%\begin{center}
% \includegraphics[width=1\textwidth]{Plots_v4_Drafts/SVD1_CoreSeconds.pdf}
\includegraphics[width=1\textwidth]{Plots_v5_Drafts/SVD1_CPUComparison.pdf}
%\end{center}
\vspace{-20pt}
\caption{
\footnotesize{Total core seconds.}}
\vspace{-10pt}
\label{fig:svd1-core-seconds}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hfill
%\hspace{-2em}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.23\textwidth}
%\begin{center}
% \includegraphics[width=1\textwidth]{Plots_v4_Drafts/SVD1_Cost.pdf}
\includegraphics[width=1\textwidth]{Plots_v5_Drafts/SVD1_CostComparison.pdf}
%\end{center}
\vspace{-20pt}
\caption{
\footnotesize{Monetary cost.}}
\vspace{-10pt}
\label{fig:svd1-cost}
\end{minipage}
\end{minipage}
\end{figure}
\end{comment}

==> sensitivity_analysis.tex <==
\vspace{-15pt}
\subsection{Sensitivity Analysis}
\label{sec:sensitivity}
\vspace{-8pt}


{\proj} is easy-to-use as it exposes only two configuration knobs to the end users---the input partition size and the number of Fargate nodes.
In this section, we discuss the results of our sensitivity analysis of these two configuration knobs.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.38\textwidth]{Plots_v3/SVD2_PartitionSizeVsRuntime.pdf}
\vspace{-10pt}
\caption{
SVD2 execution time as a function of the partition size.
}
\vspace{-10pt}
\label{fig:svd2-partitions-vs-runtime}
\end{center}
\end{figure}

\noindent\textbf{Partition Size.} 
The partition size of input data is one of the most important configuration parameters when executing a workload on {\proj}. This parameter controls how the input data is divided and subsequently processed, and presents an interesting tradeoff. Specifying a large partition size results in less parallelism and high network bandwidth consumption.
On the other hand, specifying a small partition size may generate too many fine-grained tasks, resulting in a very large number of individual connections between Task Executors and the storage cluster as well as very small data sizes for network I/O operations. Consequently, it is necessary for the user to find a balance in order to achieve optimal performance. The optimal value of the partition size will change depending on the application type and problem size. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{Plots_v3/SVD2_NumFargateNodesVsRuntime.pdf}
\vspace{-10pt}
\caption{
SVD2 performance and the I/O latencies when varying the Fargate cluster size.
}
\vspace{-15pt}
\label{fig:svd2-fargate-nodes-vs-runtime}
\end{center}
\end{figure}

Figure~\ref{fig:svd2-partitions-vs-runtime} shows the performance of SVD2 with a problem size of \(50k \times 50k\) for various partition sizes. Selecting a small partition size such as \(2k \times 2k\) causes significant network contention resulting from too many individual connections and I/O operations. Increasing the partition size alleviates this contention and improves overall performance. Notice that continuing to increase the problem size for SVD2 does not impact performance significantly. Instead, the performance will remain approximately the same as the partition size increases.  This is because task clustering and delayed I/O prevent network communication of large objects. That is, increasing the partition size does not impact the workload significantly once clustering and delay I/O are in effect.

\noindent\textbf{Number of Storage Nodes.} Next, we evaluate how the number of nodes in the storage substrate impacts execution time. Figure~\ref{fig:svd2-fargate-nodes-vs-runtime} shows the performance of SVD2 with a problem size of \(128k \times 128k\) for different numbers of Fargate nodes, along with the associated average read and write latencies for each configuration. Using a small number of nodes such as 5 or 10 results in significant performance degradation, as the limited number of Redis instances suffer severe network bandwidth contention. As we increase the size of the Fargate cluster, read latencies decrease significantly, resulting in a lower execution time for the workload.

Execution time will no longer decrease once the number of Fargate nodes increases beyond a certain threshold. The value of this threshold is predominantly dependent on problem size, as a larger problem size would benefit from a larger number of Fargate nodes compared to a smaller problem size.  
